OAG-BERT: Towards A Unified Backbone Language Model For Academic Knowledge Services

Academic knowledge services have substantially facilitated the development of the science enterprise by providing a plenitude of efficient research tools. However, many applications highly depend on ad-hoc models and expensive human labeling to understand scientific contents, hindering deployments into real products. To build a unified backbone language model for different knowledge-intensive academic applications, we pre-train an academic language model OAG-BERT that integrates both the heterogeneous entity knowledge and scientific corpora in the Open Academic Graph (OAG) -- the largest public academic graph to date. In OAG-BERT, we develop strategies for pre-training text and entity data along with zero-shot inference techniques. In OAG-BERT, we develop strategies for pre-training text and entity data along with zero-shot inference techniques. Its zero-shot capability furthers the path to mitigate the need of expensive annotations. OAG-BERT has been deployed for real-world applications, such as the reviewer recommendation function for National Nature Science Foundation of China (NSFC) -- one of the largest funding agencies in China -- and paper tagging in AMiner. All codes and pre-trained models are available via the CogDL toolkit.

==> 3_exp_summary_table.tex <==
\begin{table*}[ht]
    \centering
    \vcaption{The summary of model performance for all tasks. We report the performance of only using paper titles as inputs in \textit{title-only} and the best performance of using other features such as FOS or venue as inputs in \textit{mixed}.}
    \label{tab:exp-summary}
    \begin{threeparttable}
    \begin{tabular}{llccccccccc}
    \toprule
    \multicolumn{2}{c}{\multirow{2}{*}{Method}} & \multicolumn{3}{c}{Zero-shot Inference\footnotemark[1]} & \multicolumn{3}{c}{Supervised Classification\footnotemark[2]} & \multirow{2}{*}{NA\footnotemark[3]} & \multicolumn{2}{c}{Link Prediction\footnotemark[4]} \\
        & & FOS & Venue & Affiliation & FOS & Venue & Affiliation & & Paper-Field & Paper-Venue \\
    \midrule
    \multirow{2}{*}{SciBERT} & \textit{title-only} & 29.59\% & 10.03\% & 8.00\% & 55.13\% & 61.86\% & 35.44\% & 0.3690 & 0.4740 & 0.4570 \\
    & \textit{mixed} & 35.33\% & 18.00\% & 12.40\% & 55.63\% & 78.05\% & 56.04\% & 0.4101 & - & - \\
    \midrule
    \multirow{2}{*}{OAG-BERT} & \textit{title-only} & 37.33\% & 22.67\% & 11.77\% & 54.54\% & 63.03\% & 35.04\% & 0.4120 & \textbf{0.4892} & \textbf{0.4844} \\
    & \textit{mixed} & \textbf{49.59\%} & \textbf{39.00\%} & \textbf{21.67\%} & \textbf{64.22\%} & \textbf{78.47\%} & \textbf{57.63\%} & \textbf{0.4823} & - & - \\
    \bottomrule
    \end{tabular}
    \begin{tablenotes}
        \item[1,2] \small Hit@1 is reported for zero-shot inference and supervised classification.
        \item[3] \small NA is short for Name disambiguation. The macro pairwise f1 score is reported.
        \item[4] \small For link prediction tasks, we use pre-trained models to encode all types of nodes. Only title was provided for paper nodes. NDCG is reported.
    \end{tablenotes}
    \end{threeparttable}
\end{table*}

